Mask3D: Mask Transformer for 3D Semantic Instance Segmentation

Modern 3D semantic instance segmentation approaches predominantly rely on specialized voting mechanisms followed by carefully designed geometric clustering techniques. Building on the successes of recent Transformer-based methods for object detection and image segmentation, we propose the first Transformer-based approach for 3D semantic instance segmentation. We show that we can leverage generic Transformer building blocks to directly predict instance masks from 3D point clouds. In our model called Mask3D each object instance is represented as an instance query. Using Transformer decoders, the instance queries are learned by iteratively attending to point cloud features at multiple scales. Combined with point features, the instance queries directly yield all instance masks in parallel. Mask3D has several advantages over current state-of-the-art approaches, since it neither relies on (1) voting schemes which require hand-selected geometric properties (such as centers) nor (2) geometric grouping mechanisms requiring manually-tuned hyper-parameters (e.g. radii) and (3) enables a loss that directly optimizes instance masks. Mask3D sets a new state-of-the-art on ScanNet test (+6.2 mAP), S3DIS 6-fold (+10.1 mAP), STPLS3D (+11.2 mAP) and ScanNet200 test (+12.4 mAP).

==> abbrev_short.tex <==
@STRING{AG = "Aspect Graphs"}
@STRING{AV = "Active Vision"}

@STRING{CV = "Computer Vision"}
@STRING{Co = "Color"}

@STRING{Fa = "Face"}
@STRING{Fi = "Filter"}
@string{Ga = "Gabor"}
@string{Hi = "Histogram"}

@string{OR = "Object Recognition"}
@STRING{Refl = "Reflection and illumination"}

@string{Te = "Texture"}
@STRING{Tr = "Tracking"}


@STRING{TPAMI = "PAMI"}
@STRING{PAMI  = "PAMI"}
@STRING{IJCV  = "IJCV"}
@STRING{CVIU  = "CVIU"}
@STRING{CVGIP = "CVGIP:IU"}
@STRING{MVA   = "MVA"}
@STRING{PR    = "Pattern Recognition"}
@STRING{PRL   = "Pattern Recognition Letters"}
@STRING{IVC   = "Image and Vision Computing"}
@STRING{ML    = "Machine Learning"}

@STRING{FTCGV = "Foundations Trends Comp. Graphics Vision"}

@STRING{JSC    = "J. Sci. Comput."}

@STRING{JCN    = "J. Cog. Neurosci."}
@STRING(JEPHPP = "J. Exp. Psych.: Human Perception and Performance")
@STRING{JECP   = "J. Exp. Child Psych."}
@STRING{BBS    = "Behav. Brain Sc."}
@STRING{VR     = "Vis. Res."}
@STRING{AI     = "Art. Intell."}
@STRING{SIGMOD = "ACM SIGMOD"}

@STRING{CGA      = "Computer Graphics \& Applications"}
@STRING{PRESENCE = "Presence"}
@STRING{TCHI     = "ACM Trans. CHI"}
@STRING{CACM     = "Comm. ACM"}
@STRING{TACM     = "Trans. of the ACM"}
@STRING{TC       = "Trans. Comm."}
@STRING{TSE      = "IEEE Trans. Softw. Engin."}
@STRING{TMS      = "IEEE Trans. Math. Softw."}
@STRING{TIP      = "Trans. Image Proc."}
@STRING{TIS      = "IEICE Trans. Inf. & Syst."}
@STRING{TAC      = "IEEE Trans. Automatic Control"}
@STRING{TITS     = "TITS"}
@STRING{TVT      = "IEEE Trans. Vehic. Techn."}
@STRING{JRS      = "J. Robotic Systems"}
@STRING{AR       = "Autonomous Robots"}

@STRING{TOG      = "ACM Trans. Graphics"}

@STRING{ANNSTAT = "Annals of Statistics"}
@STRING{JC      = "J. Classif."}
@STRING{CAD     = "Cahiers de l'Analyse des Donn\'ees"}
@STRING{JMLR    = "JMLR"}

@STRING{JOE = "IEEE J. Oceanic Engineering"}

@STRING{JIVP = "JVIP"}

@STRING{SPL = "IEEE Signal Processing Letters"}

@STRING{IJCSI = "IJCSI"}


@STRING{ICCV   = "ICCV"}
@STRING{ICCV87 = "ICCV'87"}
@STRING{ICCV88 = "ICCV'88"}
@STRING{ICCV90 = "ICCV'90"}
@STRING{ICCV93 = "ICCV'93"}
@STRING{ICCV95 = "ICCV'95"}
@STRING{ICCV98 = "ICCV'98"}
@STRING{ICCV99 = "ICCV'99"}
@STRING{ICCV01 = "ICCV'01"}
@STRING{ICCV03 = "ICCV'03"}
@STRING{ICCV05 = "ICCV'05"}
@STRING{ICCV07 = "ICCV'07"}
@STRING{ICCV09 = "ICCV'09"}

@STRING{ECCV   = "ECCV"}
@STRING{ECCV90 = "ECCV'90"}
@STRING{ECCV92 = "ECCV'92"}
@STRING{ECCV94 = "ECCV'94"}
@STRING{ECCV96 = "ECCV'96"}
@STRING{ECCV98 = "ECCV'98"}
@STRING{ECCV00 = "ECCV'00"}
@STRING{ECCV02 = "ECCV'02"}
@STRING{ECCV04 = "ECCV'04"}
@STRING{ECCV06 = "ECCV'06"}
@STRING{ECCV08 = "ECCV'08"}
@STRING{ECCV10 = "ECCV'10"}

@string{CVPR   = "CVPR"}
@string{CVPR88 = "CVPR'88"}
@string{CVPR89 = "CVPR'89"}
@string{CVPR92 = "CVPR'92"}
@string{CVPR96 = "CVPR'96"}
@string{CVPR97 = "CVPR'97"}
@string{CVPR98 = "CVPR'98"}
@string{CVPR99 = "CVPR'99"}
@string{CVPR00 = "CVPR'00"}
@string{CVPR01 = "CVPR'01"}
@string{CVPR03 = "CVPR'03"}
@string{CVPR04 = "CVPR'04"}
@string{CVPR05 = "CVPR'05"}
@string{CVPR06 = "CVPR'06"}
@string{CVPR07 = "CVPR'07"}
@string{CVPR08 = "CVPR'08"}
@string{CVPR09 = "CVPR'09"}
@string{CVPR10 = "CVPR'10"}

@string{VPCVPR06 = "CVPR'06 Video Proceedings"}

@string{ACCV   = "ACCV"}
@string{ACCV06 = "ACCV'06"}
@string{ACCV07 = "ACCV'07"}

@string{ICPR   = "ICPR"}
@string{ICPR92 = "ICPR'92"}
@string{ICPR96 = "ICPR'96"}
@string{ICPR98 = "ICPR'98"}
@string{ICPR02 = "ICPR'02"}
@string{ICPR04 = "ICPR'04"}
@string{ICPR05 = "ICPR'05"}
@string{ICPR06 = "ICPR'06"}
@string{ICPR07 = "ICPR'07"}
@string{ICPR08 = "ICPR'08"}
@string{ICPR09 = "ICPR'09"}

@string{ICPRFGW = "ICPR'04 FG Net Workshop"}

@string{BMVC   = "BMVC"}
@string{BMVC91 = "BMVC'91"}
@string{BMVC98 = "BMVC'98"}
@string{BMVC99 = "BMVC'99"}
@string{BMVC00 = "BMVC'00"}
@string{BMVC01 = "BMVC'01"}
@string{BMVC02 = "BMVC'02"}
@string{BMVC03 = "BMVC'03"}
@string{BMVC04 = "BMVC'04"}
@string{BMVC05 = "BMVC'05"}
@string{BMVC06 = "BMVC'06"}
@string{BMVC07 = "BMVC'07"}
@string{BMVC08 = "BMVC'08"}
@string{BMVC09 = "BMVC'09"}
@string{BMVC10 = "BMVC'10"}

@string{BMCV02 = "Int'l Wksp. Biol. Motiv. Comp. Vis. (BMCV'02)"}

@string{DAGM   = "DAGM"}
@string{DAGM02 = "DAGM'02"}
@string{DAGM03 = "DAGM'03"}
@string{DAGM04 = "DAGM'04"}
@string{DAGM05 = "DAGM'05"}
@string{DAGM06 = "DAGM'06"}
@string{DAGM07 = "DAGM'07"}
@string{DAGM08 = "DAGM'08"}
@string{DAGM09 = "DAGM'09"}
@string{DAGM10 = "DAGM'10"}
@string{GCPR = "GCPR"}


@string{TDPVT = "3DPVT"}
@string{TDPVT06 = "3DPVT'06"}

@string{TDIM09 = "3DIM'09"}

@string{TDIMPVT = "3DIMPVT"}

@string{CAIP =   "International Conference on Analysis of Images
                                    and Patterns"}
@string{CAIP97 = "CAIP'97"}

@string{IJCAI77 = "IJCAI'77"}

@string{IJCAI = "IJCAI"}

@string{NIPS   = "NeurIPS"}
@string{NIPS97 = "NIPS'97"}
@string{NIPS01 = "NIPS'01"}
@string{NIPS02 = "NIPS'02"}
@string{NIPS03 = "NIPS'02"}
@string{NIPS06 = "NIPS'06"}

@string{ICML01 = "ICML'01"}
@string{ICML06 = "ICML'06"}

@string{ICIAP94 = "ICIAP'94"}
@string{ICIAP97 = "ICIAP'97"}

@string{ICIAR04 = "ICIAR'04"}

@string{CDC80 = "IEEE Conf. on Decision and Control"}

@string{SLCV04 = "ECCV'04 Workshop on Stat. Learn. in Comp. Vis."}

@string{TDRR = "ICCV Workshop on 3D Repr. and Recognition"}
@string{TDRR07 = "ICCV'07 Workshop on 3D Repr. for Recognition"}

@string{ICCVGIP08 = "ICCVGIP'08"}

@string{ICCVW09 = "ICCV Workshops"}

@string{POCV04 = "Workshop on Perc. Org. in Comp. Vis."}

@string{GMBV04 = "Workshop on Gener.-Model Based Vis."}

@string{WIVR04 = "Workshop on Image and Video Registr."}

@string{RMLE10 = "CVPR'09 Internet Vision Workshop"}

@string{RMLE10 = "ECCV'10 RMLE Workshop"}

@string{CVWW04 = "Comp. Vis. Winter Workshop (CVWW'04)"}

@string{FG95 = "Int. Workshop on Automatic Face and Gesture Recognition
(IWAFGR'95)"}
@string{FG96 = "Int. Conf. on Automatic Face and Gesture Recognition (FG'96)"}
@string{FG98 = "Int. Conf. on Automatic Face and Gesture Recognition (FG'98)"}
@string{FG = "Int. Conf. on Automatic Face and Gesture Recognition"}

@string{IROS   = "IROS"}
@string{IROS96 = "IROS'96"}

@string{ICRA   = "ICRA"}
@string{ICRA95 = "ICRA'95"}
@string{ICRA00 = "ICRA'00"}
@string{ICRA01 = "ICRA'01"}
@string{ICRA02 = "ICRA'02"}
@string{ICRA03 = "ICRA'03"}
@string{ICRA04 = "ICRA'04"}
@string{ICRA05 = "ICRA'05"}
@string{ICRA06 = "ICRA'06"}
@string{ICRA07 = "ICRA'07"}
@string{ICRA08 = "ICRA'08"}
@string{ICRA09 = "ICRA'09"}
@string{ICRA11 = "ICRA'11"}

@string{SIGGRAPH   = "SIGGRAPH"}
@string{SIGGRAPH94 = "SIGGRAPH'94"}
@string{SIGGRAPH97 = "SIGGRAPH'97"}
@string{SIGGRAPH99 = "SIGGRAPH'99"}
@string{SIGGRAPH03 = "SIGGRAPH'03"}
@string{SIGGRAPH04 = "SIGGRAPH'04"}
@string{SIGGRAPH05 = "SIGGRAPH'05"}
@string{SIGGRAPH06 = "SIGGRAPH'06"}
@string{SIGGRAPH07 = "SIGGRAPH'07"}
@string{SIGGRAPH08 = "SIGGRAPH'08"}
@string{SIGGRAPH09 = "SIGGRAPH'09"}
@string{SIGGRAPH10 = "SIGGRAPH'10"}

@string{CHI92 = "CHI'92"}
@string{CHI97 = "CHI'97"}

@string{ICIP   = "ICIP"}
@string{ICIP06 = "ICIP'06"}

@STRING{VR99  = "Virtual Reality '99"}
@STRING{VR00  = "Virtual Reality 2000"}

@STRING{UIST92 = "UIST'92"}
@STRING{UIST97 = "UIST'97"}

@STRING{WSCG99 = "WSCG'99"}

@STRING{ICASSP = "ICASSP"}

@string{SCIA93 = "SCIA'93"}
@string{SCIA91 = "SCIA'91"}

@string{EUROCOLT = "Europ. Conf. on Comput. Learning Theory"}

@string{IVS96 = {Intel. Vehicles Symp.'96}}
@string{IVS00 = {Intel. Vehicles Symp.'00}}
@string{IVS02 = {Intel. Vehicles Symp.'02}}
@string{IVS03 = {Intel. Vehicles Symp.'03}}
@string{IVS04 = {Intel. Vehicles Symp.'04}}
@string{IVS05 = {Intel. Vehicles Symp.'05}}
@string{IVS08 = {Intel. Vehicles Symp.'08}}
@string{IVS11 = {Intel. Vehicles Symp.'11}}

@string{WIT09 = {Int. Workshop Intel. Transp. (WIT'09)}}

@string{INES04 = {Intel. Eng. Syst. (INES'04)}}

@string{ICANN98 = {ICANN'98}}


@string{SEQS97 = {SEQS'97}}

@string{CIVR08 = "CIVR'08"}
@string{CIVR07 = "CIVR'07"}

@string{ICML = "ICML"}

@string{SPIE = "SPIE"}

@string{JFR = "Journal of Field Robotics"}

@string{PCVIA = "Photogrammetric Computer Vision and Image Analysis"}

@string{RSS = "RSS"}

@string{UAI = "UAI"}

@string{IVS = "Intel. Vehicles Symp."}

@string{ISRR = "ISRR"}

@string{ITSC = "ITSC"}

@string{AAAI = "AAAI"}

@string{RAS = "RAS"}

@string{IJRR = "IJRR"}

@string{WACV = "WACV"}

@string{ICME = "ICME"}

@string{ICLR = "ICLR"}

@string{IAS = "IAS"}

@string{ROMAN = "RO-MAN"}

@string{VCIP = "VCIP"}

@string{TCSVT = "TCSVT"}

@string{ISCAS = "ISCAS"}

@string{FutureTech = "FutureTech"}

@string{IJSR = "IJSR"}

@string{ACRA = "ACRA"}

@string{MICCAI = "MICCAI"}

@string{CSaE = "CS\&E"}

@string{RAL = "RA-L"}

@string{RAM = "RAM"}

@string{Sensors = "Sensors"}

@string{NIPSADW = "NIPS Autodiff Workshop"}

@string{RSSWDL = "RSS, Workshop on Limits and Potentials of Deep Learning in Robotics"}

@string{CoRL = "CoRL"}

@string{WACV = "WACV"}

@string{ICMR = "ICMR"}

@string{NeurIPS = "NeurIPS"}

@string{ACL = "ACL"}

@string{ThreeDV = "3DV"}
